Denoising Diffusion Probabilistic Models for Robust Image Super-Resolution in the Wild

Diffusion models have shown promising results on single-image super-resolution and other image- to-image translation tasks. Despite this success, they have not outperformed state-of-the-art GAN models on the more challenging blind super-resolution task, where the input images are out of distribution, with unknown degradations. This paper introduces SR3+, a diffusion-based model for blind super-resolution, establishing a new state-of-the-art. To this end, we advocate self-supervised training with a combination of composite, parameterized degradations for self-supervised training, and noise-conditioing augmentation during training and testing. With these innovations, a large-scale convolutional architecture, and large-scale datasets, SR3+ greatly outperforms SR3. It outperforms Real-ESRGAN when trained on the same data, with a DRealSR FID score of 36.82 vs. 37.22, which further improves to FID of 32.37 with larger models, and further still with larger training sets.

==> plot_teval_fid_40M_bigdataset.tex <==

\begin{tikzpicture}
\begin{axis}[
    title=Small Model Trained on Large Dataset,
    xlabel=$t_{eval}$,
    ylabel=FID(10k),
    xmin=0.0, xmax=0.5,
    ymin=20, ymax=40,
    xtick={0.0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5},
    xticklabels={0.0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5},
    ytick={30,40,...,100}
]
\addplot[smooth,mark=*,blue] plot coordinates {
    (0.0,37.584)
    % (0.05,33.063)
    % (0.10,32.374)
    % (0.15,32.424)
    % (0.20,33.250)
    % (0.25,34.625)
    % (0.30,35.222)
    % (0.35,35.385)
    % (0.40,36.089)
};
\addlegendentry{DRealSR}

\addplot[smooth,color=red,mark=x]
    plot coordinates {
        (0.0,27.199)
    %     (0.05,25.223)
    %     (0.10,24.317)
    %     (0.15,24.298)
    %     (0.20,24.529)
    %     (0.25,24.948)
    %     (0.30,25.682)
    %     (0.35,26.123)
    %     (0.40,26.798)
    };
\addlegendentry{RealSR}
\end{axis}
\end{tikzpicture}

==> plot_teval_fid_40M_df2kost.tex <==

\begin{tikzpicture}
\begin{axis}[
    title=Small Model Trained on Small Dataset,
    xlabel=$t_{eval}$,
    ylabel=FID(10k),
    xmin=0.0, xmax=0.5,
    ymin=20, ymax=40,
    xtick={0.0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5},
    xticklabels={0.0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5},
    ytick={30,40,...,100}
]
\addplot[smooth,mark=*,blue] plot coordinates {
    (0.0,37.584)
    % (0.05,33.063)
    % (0.10,32.374)
    % (0.15,32.424)
    % (0.20,33.250)
    % (0.25,34.625)
    % (0.30,35.222)
    % (0.35,35.385)
    % (0.40,36.089)
};
\addlegendentry{DRealSR}

\addplot[smooth,color=red,mark=x]
    plot coordinates {
        (0.0,27.199)
    %     (0.05,25.223)
    %     (0.10,24.317)
    %     (0.15,24.298)
    %     (0.20,24.529)
    %     (0.25,24.948)
    %     (0.30,25.682)
    %     (0.35,26.123)
    %     (0.40,26.798)
    };
\addlegendentry{RealSR}
\end{axis}
\end{tikzpicture}
